Elliptic flow of thermal photons and formation time of quark gluon plasma at RHIC

We calculate the elliptic flow of thermal photons from Au+Au collisions at RHIC energies for a range of values for the formation time $\tau_0$ but fixed entropy (or particle rapidity density). The results are found to be quite sensitive to $\tau_0$. The $v_2$ for photons decreases as $\tau_0$ decreases and admits a larger contribution from the QGP phase which has a smaller $v_2$. The elliptic flow coefficient for hadrons, on the other hand, is only marginally dependent on $\tau_0$.

==> reply.tex <==

 We thank the referee for his/her valuable comments. We have made 
the following modification in the manuscript in response to 
his/her comments: 


    The point raised by the referee about the role played by thermal 
photon $v_2$ in the total direct photon $v_2$ at large $p_T$ has been 
already discussed in the manuscript, but perhaps only in an indicative 
manner. We have now added a paragraph ( 4th page, paragraph number 17) 
to make the discussion more quantitative with a reference to Fig. 6 of 
Ref.[30]. We argue that theCompton+annihilation part of the prompt 
photons does not contribute to $v_2$. The fragmentation part may 
contribute a very small but positive $v_2$. These two contributions 
can also be accurately calculated using NLO pQCD. The jet-conversion 
photons may contribute a very small -ve $v_2$, and the net $v_2$ from 
last two contributions is essentially zero. We are only suggesting that, 
if it is possible, then this may bring out the sensitivity of the thermal 
photon elliptic flow to $\tau_0$.



We are attaching the revised latex file with this.
 
   We hope that we have properly addressed concern of the referee and 
that the paper can now be published in PRC (Rapid Communications). 





